Reweighted Mixup for Subpopulation Shift

Subpopulation shift exists widely in many real-world applications, which refers to the training and test distributions that contain the same subpopulation groups but with different subpopulation proportions. Ignoring subpopulation shifts may lead to significant performance degradation and fairness concerns. Importance reweighting is a classical and effective way to handle the subpopulation shift. However, recent studies have recognized that most of these approaches fail to improve the performance especially when applied to over-parameterized neural networks which are capable of fitting any training samples. In this work, we propose a simple yet practical framework, called reweighted mixup (RMIX), to mitigate the overfitting issue in over-parameterized models by conducting importance weighting on the ''mixed'' samples. Benefiting from leveraging reweighting in mixup, RMIX allows the model to explore the vicinal space of minority samples more, thereby obtaining more robust model against subpopulation shift. When the subpopulation memberships are unknown, the training-trajectories-based uncertainty estimation is equipped in the proposed RMIX to flexibly characterize the subpopulation distribution. We also provide insightful theoretical analysis to verify that RMIX achieves better generalization bounds over prior works. Further, we conduct extensive empirical studies across a wide range of tasks to validate the effectiveness of the proposed method.

==> 6_theory_proof.tex <==
\section{Proof}
In this appendix, we prove the Theorem~5.1 in Section~5. We consider the following optimization objective, which is the expected version of our weighted mixup loss (Equation~\ref{eq:weighted-loss}).
\begin{align*}
    L_n^{\IWmix}(\theta , S) = \frac{1}{n^2} \sum^{n}_{i,j=1} \E_{\lambda \sim D_{\lambda}} [\lambda w_i l(\theta, \tilde{x}_{i,j}, y_i) + (1-\lambda) w_j l(\theta, \tilde{x}_{i,j}, y_j)],
\end{align*}
where the loss function we consider is $l(\theta, x,y) = h(f_{\theta}(x)) - yf_{\theta}(x)$ and $h(\cdot)$ and $f_{\theta}(\cdot)$ for all $\theta\in \Theta$ are twice differentiable. 
We compare it with the standard weighted loss function
\begin{align*}
    L_n(\theta, S) = \frac{1}{n} \sum_{i=1}^n w_i [h(f_\theta(x_i)) - y_i f_\theta(x_i)].
\end{align*}

\begin{lemma}
\label{lm:mixup-corresponding}
The weighted mixup loss can be rewritten as 
\begin{align*}
    L_{n}^{m i x}(\theta, S)=L_{n}(\theta, S)+\sum_{i=1}^{3} \mathcal{R}_{i}(\theta, S)+\mathbb{E}_{\lambda \sim \tilde{\mathcal{D}}_{\lambda}}\left[(1-\lambda)^{2} \varphi(1-\lambda)\right],
\end{align*}
where 
$\tilde{\mathcal{D}}_{\lambda}$ is a uniform mixture of two Beta distributions, i.e., $\frac{\alpha}{\alpha+\beta}Beta(\alpha+1,\beta) + \frac{\beta}{\alpha+\beta}Beta(\beta+1,\alpha)$ and $\psi(\cdot)$ is some function with $\lim_{a\rightarrow 0}\psi(a)=0$. Moreover, 
\begin{align*}
\mathcal{R}_{1}(\theta, S)&=\frac{\mathbb{E}_{\lambda \sim \tilde{\mathcal{D}}_{\lambda}}[1-\lambda]}{n} \sum_{i=1}^{n}w_i \left(h^{\prime}\left(f_{\theta}\left(x_{i}\right)\right)-y_{i}\right) \nabla f_{\theta}\left(x_{i}\right)^{\top} \mathbb{E}_{r_{x} \sim \mathcal{D}_{X}}\left[r_{x}-x_{i}\right]\\
\mathcal{R}_{2}(\theta, S)&=\frac{\mathbb{E}_{\lambda \sim \tilde{\mathcal{D}}_{\lambda}}\left[(1-\lambda)^{2}\right]}{2 n} \sum_{i=1}^{n} w_i h^{\prime \prime}\left(f_{\theta}\left(x_{i}\right)\right) \nabla f_{\theta}\left(x_{i}\right)^{\top} \mathbb{E}_{r_{x} \sim \mathcal{D}_{X}}\left[\left(r_{x}-x_{i}\right)\left(r_{x}-x_{i}\right)^{\top}\right] \nabla f_{\theta}\left(x_{i}\right)\\
\mathcal{R}_{3}(\theta, S)&=\frac{\mathbb{E}_{\lambda \sim \tilde{\mathcal{D}}_{\lambda}}\left[(1-\lambda)^{2}\right]}{2 n} \sum_{i=1}^{n}w_i \left(h^{\prime}\left(f_{\theta}\left(x_{i}\right)\right)-y_{i}\right) \mathbb{E}_{r_{x} \sim \mathcal{D}_{X}}\left[\left(r_{x}-x_{i}\right) \nabla^{2} f_{\theta}\left(x_{i}\right)\left(r_{x}-x_{i}\right)^{\top}\right].
\end{align*}
\end{lemma}


% \begin{align*}
%     \tilde{L}_n^{mix} \coloneqq L_n(\theta, S) + \sum_{i=1}^3 R_i(\theta, S).
% \end{align*}
\begin{proof}
\label{subsec:proof-lemma-mixup}
The corresponding mixup version is 
\begin{align*}
    L_n^{\IWmix}(\theta , S) & = \frac{1}{n^2}\E_{\lambda\sim Beta(\alpha, \beta)}\sum_{i,j=1}^{n}[\lambda w_i h(f_{\theta}(\tilde{x}_{i,j}(\lambda))) - \lambda w_i y_i \\
    & \qquad \qquad  \qquad \qquad \qquad + (1-\lambda) w_j h(f_{\theta}(\tilde{x}_{i,j}(\lambda))) - (1-\lambda) w_j y_j]\\
    &= \frac{1}{n^2}\E_{\lambda\sim Beta(\alpha, \beta)}\E_{B\sim Bern(\lambda)} \sum_{i,j=1}^{n}[w_i B( h(f_{\theta}(\tilde{x}_{i,j})) -  y_i) \\
    & \qquad \qquad  \qquad \qquad \qquad + w_j(1-B) (h(f_{\theta}(\tilde{x}_{i,j})) - y_j)]\\
    & = \frac{1}{n^2}\sum_{i,j=1}^{n} \{\frac{\alpha}{\alpha+\beta} \E_{\lambda\sim Beta(\alpha+1,\beta)}w_i[h(f_{\theta}(\tilde{x}_{i,j})) -  y_i]  \\
    &\qquad \qquad \qquad \qquad \qquad + \frac{\beta}{\alpha+\beta}\E_{\lambda\sim Beta(\alpha,\beta+1)}w_j[h(f_{\theta}(\tilde{x}_{i,j})) -  y_j])\}\\
    &= \frac{1}{n} \sum_{i=1}^n w_i \E_{\lambda\sim \tilde{D}_{\lambda}} \E_{r_x\sim D_x^{w}} h(f(\theta, \lambda x_i + (1-\lambda)r_x)) - y_if(\theta, \lambda x_i + (1-\lambda) r_x)\\
    &=\frac{1}{n} \sum_{i=1}^n w_i \E_{\lambda \sim \tilde{D}_{x}}l_{\check{x}_i, y_i}(\theta),
\end{align*}
where $D_{x}^{w} = \frac{1}{n}\sum_{i=1}^n w_i \delta_i$ and $\check{x}_i = \lambda x_i +(1-\lambda) r_x$.

We let $\alpha=1-\lambda$ and $\psi_i(\alpha)=l_{\check{x}_i, y_i}(\theta)$. Then since we know $\psi_i$ is twice-differential, we have
\begin{align*}
    l_{\breve{x}_{i}, y_{i}}(\theta)=\psi_{i}(\alpha)=\psi_{i}(0)+\psi_{i}^{\prime}(0) \alpha+\frac{1}{2} \psi_{i}^{\prime \prime}(0) \alpha^{2}+\alpha^{2} \varphi_{i}(\alpha).
\end{align*}

By the proof of Lemma 3.1 in \cite{zhang2021how} we know 
\begin{align*}
    \psi_{i}^{\prime}(0)&=\left(h^{\prime}\left(f_{\theta}\left(x_{i}\right)\right)-y_{i}\right) \nabla f_{\theta}\left(x_{i}\right)^{\top}\left(r_{x}-x_{i}\right),\\
    \psi_i^{\prime \prime}(0)&=h^{\prime \prime}\left(f_{\theta}\left(x_{i}\right)\right) \nabla f_{\theta}\left(x_{i}\right)^{\top}\left(r_{x}-x_{i}\right)\left(r_{x}-x_{i}\right)^{\top} \nabla f_{\theta}\left(x_{i}\right)\\
    & \quad +\left(h^{\prime}\left(f_{\theta}\left(x_{i}\right)\right)-y_{i}\right)\left(r_{x}-x_{i}\right)^{\top} \nabla^{2} f_{\theta}\left(x_{i}\right)\left(r_{x}-x_{i}\right).
\end{align*}
\end{proof}

\begin{lemma}
\label{lm:mixup-GLM-loss}
Consider the centralized dataset, i.e., $\frac{1}{n}\sum_{i=1}^n x_i=0$, we have 
\begin{align*}
    \E_{\lambda\sim \tilde{\mathcal{D}}_{\lambda}}[L_n^{mix}(\theta, \tilde{S})] \approx L_n(\theta, S) + \frac{1}{2n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\E_{\lambda\sim \tilde{\mathcal{D}}_{\lambda}}(\frac{(1-\lambda)^2}{\lambda^2})\theta^{\top}\widehat{\Sigma}_X \theta,
\end{align*}
where $\widehat{\Sigma}_X=\frac{1}{n}\sum_{i=1}^n w_i x_i x_i^{\top}$, 
% $L_n(\theta, S) = \frac{1}{n} \sum_{i=1}^n w_i l(\theta, (x_i, y_i))$,
and the expectation is taken with respect to the randomness of $\lambda$.
\end{lemma}

\label{subsec:proof-of-mixup-GLM}
\begin{proof}
For GLM, the prediction is invariant to the scaling of the training data and thus we consider the re-scaled dataset $\tilde{S} = \{(\tilde{x}_i, y_i)\}_{i=1}^n$ where $\tilde{x}_i= \frac{1}{\lambda}(\lambda x_i + (1-\lambda)r_x)$.
For GLM the mixed stadard loss function is 
\begin{align*}
    L_n(\theta, \tilde{S}) = \frac{1}{n}\sum_{i=1}^n w_i l_{\check{x}_i, y_i}(\theta) = \frac{1}{n}\sum_{i=1}^n -w_i(y_i\tilde{x}_i^{\top}\theta - A(\tilde{x}_i^{\top}\theta)).
\end{align*}
In the proof of Lemma 3.3 in \cite{zhang2021how}, we know by taking expectation with respect to the randomness of $\lambda$ and $r_x$  we have the following second-order approximation for the GLM loss,
\begin{align*}
    \E[L_n(\theta, \tilde{S})] \approx L_n(\theta, S) + \frac{1}{2n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\E(\frac{(1-\lambda)^2}{\lambda^2})\theta^{\top}\widehat{\Sigma}_X \theta,
\end{align*}
where $\widehat{\Sigma}_X=\frac{1}{n}\sum_{i=1}^n w_i x_i x_i^{\top}$.
\end{proof}

% \begin{lemma}
% The output of the algorithm~\ref{algo:uncertainty} lies in the following hypothesis space with probability at least $1-\delta$,
% \begin{align*}
%      \mathcal{W}_{\gamma}\coloneqq \{x\rightarrow \theta^{\top}x, \text{such that } \theta \text{ satisfying } \E_{x}A^{''}(\theta^{\top}x)\theta^{\top}\Sigma_X\theta\le \gamma(\delta)\}.
% \end{align*}
% \end{lemma}
% \begin{proof}
% \label{proof-W}
% From Lemma~\ref{lm:mixup-GLM-loss} we know the second order approximation of the mixup loss is given by 
% \begin{align*}
%     \E_{\lambda\sim \tilde{\mathcal{D}}_{\lambda}}[L_n^{mix}(\theta, \tilde{S})] \approx L_n(\theta, S) + \frac{1}{2n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\E(\frac{(1-\lambda)^2}{\lambda^2})\theta^{\top}\widehat{\Sigma}_X \theta.
% \end{align*}
% We know the problem
% \begin{align}
% \label{eq:prime}
%     \min_{\theta\in \Theta} L_n(\theta, S) + \frac{C_1}{n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\theta^{\top}\widehat{\Sigma}_X \theta,
% \end{align}
% and the problem 
% \begin{equation}
% \label{eq:dual}
% \begin{aligned}
%     &\min_{\theta\in \Theta} L_n(\theta, S)  \\
%     & \text{s.t.}\quad \frac{C_1}{n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\theta^{\top}\widehat{\Sigma}_X \theta\le \gamma_1
% \end{aligned}
% \end{equation}
% are equivalent for some $\gamma_1$, i.e., we have the solution of~\eqref{eq:prime} is the same as the~\eqref{eq:dual} \cite{miettinen2012nonlinear} where $C_1=\frac{1}{2}\E(\frac{(1-\lambda)^2}{\lambda^2})$
% . Thus the solution of~\eqref{eq:prime} lies in the following hypothesis space:
% \begin{align*}
%     \{x\rightarrow \theta^{\top}x, \text{such that } \theta \text{ satisfying } \frac{C_1}{n} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\theta^{\top}\widehat{\Sigma}_X\theta \le \gamma_1\}.
% \end{align*}

% Since we know $w_iA^{''}(x_i^{\top}\theta)$ is bounded by K by Assumption~\ref{as:A}, applying Lemma~\ref{} we have 
% \begin{align*}
    
% \end{align*}
% Moreover, by Lemma~\ref{lm:concentration} we know with probability at least $1-\delta$
% \begin{align*}
%     \theta^{\top}\Sigma_X\theta &\le \theta^{\top}\hat{\Sigma_X}\theta + \lVert \hat{\Sigma}_X - \Sigma_X\rVert_{op} \lVert \theta\rVert^2 \\
%     &\le \gamma_1 + C \max \left\{\sqrt{\frac{d+\log (2 / \delta)}{n}}, \frac{d+\log (2 / \delta)}{n}\right\}\sigma^2\coloneqq \gamma(\delta).
% \end{align*}
% Thus we arrive our desired conclusions.
% % where $\zeta = \frac{1}{2} [\sum_{i=1}^n w_iA^{\prime\prime}(x_i^{\top}\theta)]\E_{\lambda\sim \tilde{\mathcal{D}}_{\lambda}}(\frac{(1-\lambda)^2}{\lambda^2})$
% % where $\tilde{x}_{i,j} = \lambda x_i + (1-\lambda) x_j$.
% % Now recall the assumption~\ref{as:A} that $K^{-1}\le \lvert A^{\prime \prime}\rvert \le K$, we get then $\zeta\ge K^{-1}$. Thus for any $\theta\in \Theta$, we have 
% \end{proof}

\begin{lemma}
\label{lm:rademacher}
Assume that the distribution of $x_i$ is $\rho$-retentive, i.e., satisfies the Assumption~\ref{as:rho-retentive}. 
Then the empirical Rademacher complexity of $\mathcal{W}_r$ satisfies 
\begin{align*}
    Rad(\mathcal{W}_r, \mathcal{S})\le \max\{(\frac{\gamma(\delta)}{\rho})^{1/4}, (\frac{\gamma(\delta)}{\rho})^{1/2}\}\cdot \sqrt{\frac{rank(\Sigma_X)}{n}},
\end{align*}
with probability at least $1-\delta$ for some constant $\gamma(\delta)$ that only depends on $\delta$.
\end{lemma}
\begin{proof}
The proof is mainly based on~\cite{zhang2021how}.
By definition, given $n$ i.i.d. Rademacher rv. $\xi_{1}, \ldots, \xi_{n}$, the empirical Rademacher complexity is
$$
\operatorname{Rad}\left(\mathcal{W}_{\gamma}, S\right)=\mathbb{E}_{\xi} \sup _{a(\theta) \cdot \theta^{\top} \Sigma_{X} \theta \leq \gamma} \frac{1}{n} \sum_{i=1}^{n} \xi_{i} \theta^{\top} x_{i}
$$
Let $\tilde{x}_{i}=\Sigma_{X}^{\dagger / 2} x_{i}, a(\theta)=\mathbb{E}_{x}\left[A^{\prime \prime}\left(x^{\top} \theta\right)\right]$ and $v=\Sigma_{X}^{1 / 2} \theta$, then $\rho$-retentiveness condition implies $a(\theta)^{2} \geq \rho \cdot \min \left\{1, \mathbb{E}_{x}\left(\theta^{\top} x\right)^{2}\right\} \geq \rho \cdot \min \left\{1, \theta^{\top} \Sigma_{X} \theta\right\}$ and therefore $a(\theta) \cdot \theta^{\top} \Sigma_{X} \theta \leq \gamma$ implies that $\|v\|^{2}=\theta^{\top} \Sigma_{X} \theta \leq \max \left\{\left(\frac{\gamma}{\rho}\right)^{1 / 2}, \frac{\gamma}{\rho}\right\}$.

As a result,
$$
\begin{aligned}
\operatorname{Rad}\left(\mathcal{W}_{\gamma}, S\right) &=\mathbb{E}_{\xi} \sup _{a(\theta) \cdot \theta^{\top} \Sigma_{X} \theta \leq \gamma} \frac{1}{n} \sum_{i=1}^{n} \xi_{i} \theta^{\top} x_{i} \\
&=\mathbb{E}_{\xi} \sup _{a(\theta) \cdot \theta^{\top} \Sigma_{X} \theta \leq \gamma} \frac{1}{n} \sum_{i=1}^{n} \xi_{i} v^{\top} \tilde{x}_{i} \\
& \leq \mathbb{E}_{\xi} \sup _{\|v\|^{2} \leq\left(\frac{\gamma}{\rho}\right)^{1 / 2} \vee \frac{\gamma}{\rho}} \frac{1}{n} \sum_{i=1}^{n} \xi_{i} v^{\top} \tilde{x}_{i} \\
& \leq \frac{1}{n} \cdot\left(\frac{\gamma}{\rho}\right)^{1 / 4} \vee\left(\frac{\gamma}{\rho}\right)^{1 / 2} \cdot \mathbb{E}_{\xi}\left\|\sum_{i=1}^{n} \xi_{i} \tilde{x}_{i}\right\| \\
& \leq \frac{1}{n} \cdot\left(\frac{\gamma}{\rho}\right)^{1 / 4} \vee\left(\frac{\gamma}{\rho}\right)^{1 / 2} \cdot \sqrt{\mathbb{E}_{\xi}\left\|\sum_{i=1}^{n} \xi_{i} \tilde{x}_{i}\right\|^{2}} \\
& \leq \frac{1}{n} \cdot\left(\frac{\gamma}{\rho}\right)^{1 / 4} \vee\left(\frac{\gamma}{\rho}\right)^{1 / 2} \cdot \sqrt{\sum_{i=1}^{n} \tilde{x}_{i}^{\top} \tilde{x}_{i}}
\end{aligned}
$$
Consequently,
$$
\begin{aligned}
\operatorname{Rad}\left(\mathcal{W}_{\gamma}, S\right)=\mathbb{E}_{S}\left[\operatorname{Rad}\left(\mathcal{W}_{\gamma}, S\right)\right] & \leq \frac{1}{n} \cdot\left(\frac{\gamma}{\rho}\right)^{1 / 4} \vee\left(\frac{\gamma}{\rho}\right)^{1 / 2} \cdot \sqrt{\sum_{i=1}^{n} \mathbb{E}_{x_{i}}\left[\tilde{x}_{i}^{\top} \tilde{x}_{i}\right]} \\
& \leq \frac{1}{\sqrt{n}} \cdot\left(\frac{\gamma}{\rho}\right)^{1 / 4} \vee\left(\frac{\gamma}{\rho}\right)^{1 / 2} \cdot \operatorname{rank}\left(\Sigma_{X}\right)
\end{aligned}
$$
Based on this bound on Rademacher complexity, Theorem ~\ref{thm:generalization} can be proved by directly applying the Theorem 8 from \cite{bartlett2002rademacher}.
\end{proof}

% \begin{lemma}[Concentration of the Covariance Matrix \cite{tropp2015introduction}]
% \label{lm:concentration}
% Let $\mathbf{x}_{1}, \ldots, \mathbf{x}_{n}$ be an i.i.d sequence of $\sigma$ sub-gaussian random vectors such that $\mathbb{V}\left[\mathbf{x}_{1}\right]=\Sigma$ and let $\hat{\Sigma}_{n}:=\frac{1}{n} \sum_{i=1}^{n} x_{i} x_{i}^{T}$ be the empirical covariance matrix. Then there exists a universal constant $C>0$ such that, for $\delta \in(0,1)$, with probability at least $1-\delta$
% $$
% \frac{\left\|\hat{\Sigma}_{n}-\Sigma\right\|_{o p}}{\sigma^{2}} \leq C \max \left\{\sqrt{\frac{d+\log (2 / \delta)}{n}}, \frac{d+\log (2 / \delta)}{n}\right\}.
% $$
% \end{lemma}

==> abstract.tex <==
Subpopulation shift exists widely in many real-world applications, which refers to the training and test distributions that contain the same subpopulation groups but with different subpopulation proportions. Ignoring subpopulation shifts may lead to significant performance degradation and fairness concerns. Importance reweighting is a classical and effective way to handle the subpopulation shift. However, recent studies have recognized that most of these approaches fail to improve the performance especially when applied to over-parameterized neural networks which are capable of fitting any training samples. In this work, we propose a simple yet practical framework, called reweighted mixup (RMIX), to mitigate the overfitting issue in over-parameterized models by conducting importance weighting on the ''mixed'' samples. Benefiting from leveraging reweighting in mixup, RMIX allows the model to explore the vicinal space of minority samples more, thereby obtaining more robust model against subpopulation shift. When the subpopulation memberships are unknown, the training-trajectories-based uncertainty estimation is equipped in the proposed RMIX to flexibly characterize the subpopulation distribution. We also provide insightful theoretical analysis to verify that RMIX achieves better generalization bounds over prior works. Further, we conduct extensive empirical studies across a wide range of tasks to validate the effectiveness of the proposed method.
